Real-Time Scheduling of Machine Learning Operations on Heterogeneous Neuromorphic SoC

Neuromorphic Systems-on-Chip (NSoCs) are becoming heterogeneous by integrating general-purpose processors (GPPs) and neural processing units (NPUs) on the same SoC. For embedded systems, an NSoC may need to execute user applications built using a variety of machine learning models. We propose a real-time scheduler, called PRISM, which can schedule machine learning models on a heterogeneous NSoC either individually or concurrently to improve their system performance. PRISM consists of the following four key steps. First, it constructs an interprocessor communication (IPC) graph of a machine learning model from a mapping and a self-timed schedule. Second, it creates a transaction order for the communication actors and embeds this order into the IPC graph. Third, it schedules the graph on an NSoC by overlapping communication with the computation. Finally, it uses a Hill Climbing heuristic to explore the design space of mapping operations on GPPs and NPUs to improve the performance. Unlike existing schedulers which use only the NPUs of an NSoC, PRISM improves performance by enabling batch, pipeline, and operation parallelism via exploiting a platform's heterogeneity. For use-cases with concurrent applications, PRISM uses a heuristic resource sharing strategy and a non-preemptive scheduling to reduce the expected wait time before concurrent operations can be scheduled on contending resources. Our extensive evaluations with 20 machine learning workloads show that PRISM significantly improves the performance per watt for both individual applications and use-cases when compared to state-of-the-art schedulers.

==> sections/results_old.tex <==
\subsection{Throughput}
Figure~\ref{fig:throughput} plots the throughput of each evaluated mechanism for our evaluated machine learning workloads. All results are normalized to the throughput obtained using the baseline mechanism.
We make the following three key observations.

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/throughput.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Throughput normalized to Baseline.}
	%\vspace{-10pt}
	\label{fig:throughput}
\end{figure}

\begin{figure*}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=1.99\columnwidth]{images/improvements.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Throughput of SDFG of Figure~\ref{fig:sdfg_example}(a) obtained using \dfs{}~\cite{dfsynthesizer_pp}, baseline (MetaTF)~\cite{metatf}, SentryOS~\cite{sentryos}, and the proposed design flow.}
	%\vspace{-10pt}
	\label{fig:improvements}
\end{figure*}

First, between baseline and \dfs{}, throughput obtained using the baseline is on average 1.7x higher than \dfs{}. Second, throughput using \sos{} is 1.3x lower than baseline but 31\% higher than \dfs{}. Finally, throughput using the proposed design flow is the highest among all evaluated mechanism (on average, 6.1x higher than baseline, 9.2x higher than \dfs{}, and 7.1x higher than \sos{}). To provide insight to these improvements, Figure~\ref{fig:improvements} illustrates the schedules constructed using the four mechanism for the SDFG shown in Figure~\ref{fig:sdfg_example}(a).
We observe that even though both \dfs{} and baseline do not enable pipelining, the period of \dfs{} is higher than baseline because of the increased latency of operations scheduled on the GPP. Therefore, the throughput of \dfs{} is lower than baseline.
\sos{}, on the other hand enables pipelining. So, its period is lower than \dfs{} (throughput is higher than \dfs{}). 
However, the latency of operations on the GPP is still high. So, the throughput is lower than the baseline.
Finally, the proposed design flow exploits the heterogeneity of the hardware efficiently using the Hill Climbing heuristic.
It exploits pipelining and data-level parallelism using its block scheduling approach.
So, it period is the lowest, i.e., throughput is the highest among all evaluated mechanisms.

\subsection{Energy-per-Inference}

\subsection{Use-case Mapping}

\subsection{Compilation Time and Run-time Overhead}

\subsection{Hill Climbing Initial Mapping Selection}

\subsection{Performance Scaling}
Figure~\ref{fig:scaling} plots the throughput obtained using the proposed design flow (normalized to baseline) as the number of NPUs is increased from 80 (Akida) to 128 (Loihi). We make the following two key observations.

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/scaling.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Throughput normalized to Baseline.}
	%\vspace{-10pt}
	\label{fig:scaling}
\end{figure}

First, the throughput scaling is proportional to the number of NPUs (i.e., 1.6x) for LeNet, AlexNet, and VGG16.
This is because these models have chain-like connections with convolutions and pooling operations. There is a limited amount of parallelism that exists within their model structure.
Therefore, the proposed design flow can only improve throughput by processing multiple iterations in parallel (limited by the number of NPUs).
Second, for all other models, the proposed design flow exploits the parallelism in their model structure in addition to executing iterations on the parallel NPUs. The average improvement for these models is 2.2x.

==> sections/scheduler.tex <==
Scheduling SDCNN operations on an \nsoc{} platform consists of the following three steps --- mapping, ordering, and timing~\cite{SB00}.
Mapping involves assigning operations to different computing units of an \nsoc{} platform.
Ordering involves determining execution order of operations mapped to each computing unit of the platform.
Finally, timing involves determining the start time of each operation on the computing unit to which it is mapped. 
These steps can be performed during compile time or at run-time.

We focus on compile time scheduling techniques.
We enable self-timed execution and ordered transaction strategy~\cite{lee1989scheduling}.
In real-time scheduling theory, self-timed execution refers to an approach where each computing unit executes the operations assigned to it in a fixed order that is specified at compile time.
Before executing an operation, a computing unit must wait for all the data needed to perform the operation.
In this way, run-time synchronizations are enforced.
Self-time execution eliminates the timing step of the scheduling as postulated above. 
It also provides robustness when the execution time of an operation may occasionally deviate at run-time.
The ordered transaction strategy is to add communication actors at compile time to model the handshaking of data between two computing units where a pair of communicating operations are mapped.
This transaction order of data communication is then enforced at run-time.
Figure~\ref{fig:iterative_scheduling} illustrates at a high-level our iterative mapping and ordering of SDCNN operations exploiting a graph-theoretic intermediate representation and using self-timed execution (STE) and ordered transaction strategy (OTS). 
%We now describe these steps in details.

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.9\columnwidth]{images/overview.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Iterative mapping and ordering of operations.}
	%\vspace{-10pt}
	\label{fig:iterative_scheduling}
\end{figure}



\begin{figure*}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=1.99\columnwidth]{images/scheduling_demo.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{AScheduling of the projection block of ResNet with four different operations -- pooling, convolution, batch normalization (BN), and addition. (a) NPU-only scheduling of operations using existing software framework such as MetaTF. (b) Proposed scheduling where we exploit the heterogeneity of the platform in scheduling operations. (c) NPU-only scheduling where the NPU does not have the hardware to accelerate the BN operation. (d) Proposed scheduling for the same type of NPU (i.e., with BN acceleration). Reductions in the execution time are highlighted in this figure as improvements.}
	%\vspace{-10pt}
	\label{fig:scheduling_demo}
\end{figure*}

\begin{figure*}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=1.99\columnwidth]{images/ordering_new.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{(a) An SDFG and its mapping. (b) Mapping-aware SDFG (IR). (c) Ordering of actors of the IR using Max-Plus Algebra. (d) Proposed IR with operations organized according to the individual units to which they are mapped. (e) Overlapped schedule with multiple iterations pipelined in the hardware.}
	%\vspace{-10pt}
	\label{fig:ordering}
\end{figure*}


\subsection{Mapping Operations}
To formulate the mapping, i.e., operation assignment problem, we first introduce the following notations.
Here, an SDCNN model is considered to be a collection of layers, where each layer performs a specific operation. 
For instance, the CONV layer in Figure~\ref{fig:sdfg_example}(a) performs the convolution operation on the units (neurons) of the pooling (POOL) layer.

\begin{footnotesize}
\begin{align*}
G_\text{SDCNN}(L,C) &=~\text{An SDCNN application}\\
L &=~\text{Set of layers of the application and } |L| = N_L\\
C &=~\text{Connection between layers}\\
G_{\nsoc{}}(U,E) &=~\text{An NSoC platform}\\
U &=~\text{Set of computing units of the \nsoc{} and } |U| = N_U\\
E &=~\text{Edges/links between the computing units}\\
\mathcal{M} &=~\{x_{i,j}\} =~\text{Mapping of }G_\text{SDCNN} \text{ on } G_{\nsoc{}} \\
x_{i,j} =& \begin{cases}
1 & \text{if layer } L_i\in {L} \text{ is assigned to computing unit } U_j\in U\\
0 & \text{otherwise}
\end{cases}
\end{align*}
\end{footnotesize}
\normalsize

Determining the mapping, i.e., assignment of operations to the computing units of an \nsoc{} involves solving for the variables \ineq{x_{i,j}} such that an objective function is
minimized.
In this work, throughput is the performance metric defined as the inverse of the maximum cycle mean (Eq.~\ref{eq:perf_def}). Therefore, the objective function is to minimize the maximum cycle mean (i.e., the period).
Doing so, maximizes the throughput.
%(speedup in this case) is optimized (maximized). 
%We define and formulate the optimization objective in Sec.~\ref{sec:ordering}.

The problem we aim to solve draws parallel to finding mapping of tasks to parallel computers~\cite{singh2013mapping}. 
This problem has been shown to be NP-complete for non-trivial optimization objectives~\cite{rosenberg1978data}.
Therefore, heuristic solutions such as Hill Climbing, Simulated Annealing, and Genetic Algorithms are shown to be effective in finding an optimum mapping~\cite{talbi1993hill}.
We use a Hill Climbing heuristic because of its simplicity~\cite{smitley1988comparative} and possible application to run-time scheduling~\cite{fattah2013smart}.

Figure~\ref{fig:hill_climbing_demo} illustrates the steps for the proposed Hill Climbing heuristic.
%The corresponding pseudo-code is shown as Algorithm~\ref{algo:hill_climbing_demo}.
The heuristic starts with the \emph{generate initial mapping} block, 
%(line x in Algorithm~\ref{algo:hill_climbing_demo}).
%This block 
which generates a set of initial mappings.
One of these mappings is selected as the starting mapping and the heuristic proceeds to the exploration stage (see Section~\ref{sec:initial_mapping_selection} for initial mapping selection).
In the exploration stage, the heuristic performs trial swaps for each layer \ineq{L_i\in L} with other layers that are mapped to different computing units of the \nsoc{} platform.
A trial swap operation involves changing the mapping matrix temporarily, as we illustrate to the right of the figure.
For each of these trial swaps, the heuristic evaluates the optimization objective and selects the one that leads to the highest improvement in the objective function.
In case of a tie, it selects a trial swap randomly.
Once a swap is finalized, it makes the swap permanent by updating the mapping.
The heuristic then iterates through the steps for the next layer.

A pass in this heuristic consists of performing trial swaps for every pair of layers that are mapped to different computing units in a given mapping.
If during a pass, the objective function improves, then another pass of the heuristic is performed.
Otherwise, the heuristic is said to be stuck at a local minimum.
To come out of this local minimum, the mapping is perturbed.
This involves performing a fixed number of random swaps and restarting the iterative procedure.

\subsubsection{Initial Mapping Selection}\label{sec:initial_mapping_selection}
We show that the choice of initial mapping critically influences the performance of the Hill Climbing heuristic.
We evaluate the following three initial mapping selection techniques.
\begin{enumerate}
    \item \textbf{Random (Rnd):} Here, operations are randomly distributed to computing units.
    \item \textbf{Load-Balance (LB):} Here, operations are distributed equally amongst the computing units.
    \item \textbf{NPU-First Mapping (NFM):} Here, operations are assigned on a first-ready-first-serve basis to the first available unit, prioritizing an NPU over a CPU.
\end{enumerate}

\subsection{Performance Improvement Opportunity}
To understand how the Hill Climbing heuristic is able to improve performance, we consider the example of scheduling the operations in the projection block of ResNet on the \nsoc{} platform.
Figure~\ref{fig:scheduling_demo}(a) presents the schedule created by existing system software like MetaFF~\cite{metatf}, which utilizes only the NPU of the platform to execute these operations.
Figure~\ref{fig:scheduling_demo}(b) shows the schedule created by the proposed Hill Climbing heuristic (and operation ordering, which we explain in Section~\ref{sec:ordering}).
Here, both the GPP and NPU are used to exploit the parallelism in the SDFG representation of the projection block.
By doing so, we reduce the time it takes to complete the execution of this block.
Here, we also illustrate data communications on the shared interconnect.

Now, imagine that the NPU does not have the hardware to accelerate batch normalization. The baseline MetaTF cannot schedule ResNet.
However, one simple modification is where only the batch normalization is scheduled on the GPP and all other operations on the NPU.
The corresponding scheedule is shown in Figure~\ref{fig:scheduling_demo}(c).
We show that even for such NPUs, which do not support a few operations (batch normalization in this example), execution time can be significantly reduced by efficiently scheduling operations using our design flow as we illustrate in Figure~\ref{fig:scheduling_demo}(d).

\subsection{Ordering Operations}\label{sec:ordering}
To obtain the ordering of operations on computing units, our design methodology is the following.
We start with an SDFG and mapping of this SDFG to the \nsoc{} platform using the Hill Climbing heuristic. This is shown in Figure~\ref{fig:ordering}(a).
Next, we construct a mapping-aware SDFG, which is an intermediate representation (IR).
This is shown in Figure~\ref{fig:ordering}(b).
This IR consists of actors that represent data communication (shown with grayed circles).
Therefore, this IR is a type of inter-process communication (IPC) graph.
In creating this IR, the execution time of an actor is updated to its latency on the computing unit where it is mapped.
Finally, we use the Max-Plus formulation of Section~\ref{sec:performance} to compute the execution end times of actors (Eq.~\ref{eq:laeqn}). 
The maximum cycle mean is then computed using Equation~\ref{eq:mcm} and the throughput using Equation~\ref{eq:perf_def}.
The period of this schedule is indicated as \ineq{P}.
%To use this strategy, the interconnect latency behavior must be known at compile time. 
%We show that such behavior can be predicted to a reasona

% \begin{figure}[h!]
% 	\centering
% 	%\vspace{-5pt}
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/ordering.pdf}}
% 	%\vspace{-10pt}
% 	%\caption{An example of spiking neural network.}
% 	\caption{(a) An SDFG and its mapping. (b) Mapping-aware SDFG (IR). (c) Ordering of actors of the IR using Max-Plus Algebra.}
% 	%\vspace{-10pt}
% 	\label{fig:ordering}
% \end{figure}

Ordering operations on an \nsoc{} platform draws parallel to scheduling tasks on a multiprocessor system with GPPs.
A key difference is that unlike a GPP, the internal architecture of an NPU consists of individual hardware units to accelerate different SDCNN operations.
Therefore, pipelining can be enabled inside the NPU to perform operations from different iterations in parallel.
To facilitate such overlapped execution, we propose to extend the IR of Figure~\ref{fig:ordering}(b) with an IPC graph where operations are organized according to the individual units to which they are mapped.
We call this heterogeneous IR (hIR).
An hIR of the IR in Figure~\ref{fig:ordering}(b) is illustrated in Figure~\ref{fig:ordering}(d). 
We note that operations that communicate with one another and are mapped within the NPU (e.g., actors \ineq{\actor{a}_0} and \ineq{\actor{a}_3}) do not introduce any communication actors because the data communication takes place using dedicated low-latency channels within the NPU (see Figure~\ref{fig:nsoc}).
%compared to when they are mapped to the CPU and NPU (e.g., actors \ineq{\actor{a}_0} and \ineq{\actor{a}_3}).

% \begin{figure}[h!]
% 	\centering
% 	%\vspace{-5pt}
% 	\centerline{\includegraphics[width=0.99\columnwidth]{images/oveerlapped_ordering.pdf}}
% 	%\vspace{-10pt}
% 	%\caption{An example of spiking neural network.}
% 	\caption{(a) Proposed IR with operations organized according to the individual units to which they are mapped. (b) Overlapped schedule with multiple iterations pipelined in the hardware.}
% 	%\vspace{-10pt}
% 	\label{fig:overlapped_ordering}
% \end{figure}

To construct the overlapped (pipelined) scheduling of iterations, we propose a block scheduling mechanism, where \ineq{N} iterations of the SDFG, each represented as an hIR, are combined together as a single SDFG block. 
This block is then scheduled using the Max-Plus algebraic formulation of Section~\ref{sec:performance}. Figure~\ref{fig:ordering}(e) shows the overlapped schedule.
The period of this schedule is \ineq{P_b}.
We can clearly see that \ineq{P_b < P}.
Therefore, the block scheduler reduces the period, i.e., improves the throughput by creating opportunities for pipelining and exploiting data-level parallelism.

Once the firing end times of actors in the block schedule are obtained, the timing information is discarded, retaining only the order in which actors need to fire on each computing unit. This is to enable self-timed execution. As the constructed schedule also involves communication actors, ordered transaction strategy is also enforced in the scheduling.

% In Section~\ref{sec:ordering}, we discuss block scheduling technique, which overlaps the execution of multiple iterations of an SDFG to significantly improve throughput.

Algorithm~\ref{alg:ordering} shows the pseudo-code of the scheduling.
While lines 1-14 define the Hill Climbing heuristic (of Figure~\ref{fig:hill_climbing_demo}).
Lines 15-20 define the procedure to compute the block schedule and compute the period.
Here, the original application SDFG is converted into a mapping-aware SDFG (IR) as illustrated in Figure~\ref{fig:ordering}(b). 
Next, the heterogeneous IR is constructed by exploiting the platform's heterogeneity. This is illustrated in Figure~\ref{fig:ordering}(d).
Next, a block SDFG is constructed \ineq{N} iterations.
Finally, the block period is computed using the Max-Plus formulation of Eq.~\ref{eq:perf_def}.

\begin{algorithm}[h]
	\scriptsize{
 		\KwIn{\ineq{G_\text{SDCNN}(\textbf{L},\textbf{C})},\ineq{G_{\nsoc}(\textbf{U},\textbf{E})}}
 		%\KwOut{\ineq{G_{DFG}= (\textbf{S},\textbf{C})}}
 		$\mathcal{M}_\text{init} = \texttt{generate\_initial\_mapping}(G_\text{SDCNN},G_\nsoc{})$\tcc*[r]{Generate initial mapping}
 		$P_\text{init} = \texttt{GenerateSchedule}(G_\text{SDCNN},G_\nsoc{},\mathcal{M}_\text{init})$\tcc*[r]{Compute the block period of this mapping}
 		\For(\tcc*[f]{For each layer}){$\l_i \in L$}{
 		    \For(\tcc*[f]{For other layers not mapped to the same computing unit}){$l_j\in L \text{ and } x_{i,k} \neq x_{j,k}\forall k $}{
 		        $\mathcal{M}_\text{temp} = \texttt{swap}(\mathcal{M}_\text{init},i,j)$\tcc*[r]{Swap the mapping.}
 		        $P_b = \texttt{GenerateSchedule}(G_\text{SDCNN},G_\nsoc{},\mathcal{M}_\text{temp})$\tcc*[r]{Compute the block period.}
 		        $P.\texttt{append}(P_b) \text{ and } M.\texttt{append}(\mathcal{M}_\text{init})$\tcc*[r]{Save the mapping and the schedule.}
 		    }
 		    $x = \texttt{argmin}(P)$\tcc*[r]{Find the index to the minimum period.}
 		    \If(\tcc*[f]{If the period improves.}){$P[x] < P_\text{init}$}{
 		        $P_\text{init} = P[x]$ and
 		        $\mathcal{M}_\text{init} = M[x]$\tcc*[r]{Make the swap permanent and update the schedule.}
 		    }
 		}
 		\uIf(\tcc*[f]{If the pass reduces period.}){\text{pass is successful}}{
 		    Repeat steps 3-10\tcc*[r]{Pass is successful and the steps 3-10 are repeated.}
 		}
 		\Else(\tcc*[f]{If there is no improvement, the algorithm is stuck at a local minimum.}){
 		    $\mathcal{M}_\text{init} = \texttt{Perturb}$
 		    Repeat steps 3-10\tcc*[r]{Perturb the mapping by randomly swapping the allocation and the Hill Climbing pass is repeated.}
 		}
 		\Def(\tcc*[f]{Procedure to generate the schedule.}){$\texttt{GenerateSchedule}(G_\text{A},G_\text{P},\mathcal{M})$}{
 		    $G_\text{IR} = \texttt{Transform}(G_\text{A},G_\text{P},\mathcal{M})$\tcc*[r]{Convert the SDFG to mapping-aware SDFG (IR). See Figure~\ref{fig:ordering}(b).}
 		     $G_\text{hIR} = \texttt{HeterogeneousIR}(G_\text{IR},G_\text{P})$\tcc*[r]{Convert to heterogeneous IR by exploiting a platform's heterogeneity. See Figure~\ref{fig:ordering}(d).}
 		     $G_\text{Block} = \texttt{BlockSDFG}(G_\text{hIR},N)$\tcc*[r]{Create block SDFG combining $N$ iterations.}
 		     $P_b = \texttt{MaxPlus}(G_\text{Block})$\tcc*[r]{Compute the block period using the Max-Plus formulation of Eq.~\ref{eq:perf_def}.}
 		     $\texttt{return} P_b$
 		}
 		
 	}
	\caption{\footnotesize{Ordering of operations on computing units.}}
	\label{alg:ordering}
\end{algorithm}


==> sections/sdfg_old.tex <==
\subsection{Synchronous Dataflow Graphs}
Synchronous Data Flow Graphs (SDFGs, see \cite{sdfg}) are commonly used to model streaming applications that are implemented on a multi-processor system-on-chip~\cite{SB00}. Both pipelined streaming and cyclic dependencies between tasks can be easily modeled in SDFGs. These graphs are used to analyze a system in terms of throughput and other performance properties, e.g., execution time and buffer requirements~\cite{Stuijk06dac}. 

Nodes of an SDFG are called \textit{actors}. 
%Each node is a cluster of the SNN. 
Actors are computed by reading \textit{tokens} (spikes) from their input ports and writing results of their computation as tokens on output ports. The number of tokens produced or consumed in one execution of an actor is called the \textit{port rate}. 
%They represent the number of spikes per unit time at the input and output of different clusters in the SNN. 
Port rates are visualized as annotations on edges. Actor execution is also called \textit{firing}, and it requires a fixed amount of time to execute on a computing unit. Edges in the graph are called \textit{channels} and they represent dependencies among actors.

An actor is called {\em ready} when it has sufficient input tokens on all its input channels and sufficient buffer space on all its output channels; an actor can only fire when it is ready.

\begin{Definition}{Actor}
{An actor $\actor{a}_i$ is a tuple $(I_i,O_i,\tau_i,\mu_i)$ consisting of a set $I_i$ ($\subseteq Ports$) of input ports, a set $O_i$ ($\subseteq Ports$) of output ports with $I_i \cap O_i = \emptyset$, $\tau_i$ is the execution time of $\actor{a}_i$ and $\mu_i$ is its state space, which represents weights.}
%$\tau \in \mathbb{N}\setminus\{0\}$ representing the execution time of a ($\tau(a)$).}
\end{Definition}

\begin{Definition}{SDFG}
{An SDFG is a directed graph $G = (A,C)$ consisting of a finite set $A$ of actors and a finite set $C\subseteq Ports^2$ of channels. The source of channel $ch_i^j \in C$ is an output port of actor $\actor{a}_i$, the destination is an input port of actor $\actor{a}_j$. All ports of all actors are connected to precisely one channel, and all channels are connected to ports of some actors. The source and the destination port of channel $ch_i^j$ are denoted by $SrcP(ch_i^j)$ and $DstP(ch_i^j)$ respectively. Channels connected to the input and output ports of an actor $\actor{a}_i$ are denoted by $InC(\actor{a}_i)$ and $OutC(\actor{a}_i$) respectively.}
\end{Definition}

Before an actor $\actor{a}_i$ starts its firing, it requires $Rate(q_i)$ tokens from all $(p,q_i)\in InC(\actor{a}_i)$. When the actor completes execution, it produces $Rate(p_i)$ tokens on every $(p_i,q) \in OutC(\actor{a}_i)$. One important property of an SDFG is \textit{throughput}, which is defined as the inverse of its long-term period. A period is the average time needed for one iteration of the SDFG. An iteration is defined as the minimum non-zero execution such that the original state of the SDFG is obtained. 
This is the performance parameter used in this paper.
In Section~\ref{sec:ordering}, we modify this definition to incorporate pipelining.

\subsection{Performance Estimation}\label{sec:performance}
The long-term throughput of an SDFG can be computed by analyzing its maximum cycle mean (MCM). 
We use Max-Plus Algebra \cite{heidergott2014max}, a real-time calculus to compute the MCM.
The Max-Plus semiring \ineq{\mathbb{R}_{\text{max}}} is the set \ineq{\mathbb{R}\cup\{-\infty\}} defined with two basic operations \ineq{\oplus \text{ and } \otimes} that are related to linear algebra as
\begin{equation}
\label{eq:mpb}
\footnotesize a \oplus b = \max(a,b) \text{  and  } a \otimes b = a + b.
\end{equation}
The identity element \ineq{\mymathbb{0}} for the addition \ineq{\oplus} is \ineq{-\infty} in linear algebra, i.e., \ineq{a \oplus \mymathbb{0} = a}. The identity element \ineq{\mymathbb{1}} for the multiplication \ineq{\otimes} is 0 in linear algebra, i.e., \ineq{a \otimes \mymathbb{1} = a}.

To use Max-Plus Algebra in analyzing an SDFG, it is customary to express the time at which an actor fires in terms of preceding firings in linear algebra and then use standard analysis techniques for Max-Plus Algebra to estimate timing performance. We use the running example of a portion of the SDFG representing only the projection block of ResNet shown in Figure~\ref{fig:sdfg_example}(a). 
%which represents the projection block of ResNet.
The corresponding SDFG is shown in Figure~\ref{fig:sdfg_example}(b). 
This is the SDFG representation for one invocation (iteration) of the ResNet model, performing classification of the image presented to its input.
In the context of (iterative) streaming applications, this SDFG will be applied to each image successively.
We illustrate the \ineq{(k-1),k,} and \ineq{(k+1)^{\text{th}}} iteration of the SDFG in Figure~\ref{fig:sdfg_example}(c).
The firing end times of all eight actors in the $k^{\text{th}}$ iteration (in linear algebra) are 

\begin{footnotesize}
\begin{align}
\label{eq:laeqn}
t_{0}(k) &\ge t_{0}(k-1) + \tau_{0} & 
t_{4}(k) &\ge t_{3}(k) + \tau_{4}\\
%\texttt{max}\Big[t_{2}(k),t_{1}(k),t_{4}(k)\Big] + \tau_5\\
t_{1}(k) &\ge t_{0}(k) + \tau_1 & 
t_{5}(k) &\ge t_{4}(k) + \tau_5\nonumber\\
t_{2}(k) &\ge t_{1}(k) + \tau_2 & 
t_{6}(k) &\ge t_{5}(k) + \tau_6\nonumber\\
t_{3}(k) &\ge t_{0}(k) + \tau_3 & 
t_{7}(k) &\ge \texttt{max}\Big[t_{2}(k),t_{6}(k)\Big] + \tau_7\nonumber
%\max\Big[t_3(k-1),t_5(k-1),t_{2}(k),t_{4}(k),t_{6}(k)\Big] + \tau_{1}\nonumber\\
%t_{4}(k) &\ge \texttt{max}\Big[t_{1}(k),t_{0}(k)\Big] + \tau_4 \nonumber
\end{align}
\end{footnotesize}\normalsize

where a subscript indicate the actor number.
Observe that the firing end time of actor \ineq{\actor{a}_0} in the  \ineq{k^\text{th}} iteration is after its firing end time in the \ineq{(k-1)^\text{th}} iteration. 
Since each actor represents a layer of an SDCNN model (see Figure~\ref{fig:sdfg_example}), the production and consumption rates are the same for every channel in the SDFG. This is to ensure that the tokens (spikes) communicated from a source layer to its destination are consumed entirely within the iteration.
%layer is specific to the image being processed by the model. 
Using previously introduced Max-Plus semantics, firing end times for every actor in the SDFG  can be expressed as
\begin{equation}
\label{eq:mat}
\footnotesize\mathbf{t_k} = \oplus\mathbf{{T}\otimes t_{k-1}}
\end{equation}
where $\mathbf{{T}}$ is a matrix in \ineq{\mathbb{R}_{\text{max}}^{8\times 8}} that captures the actor execution times $\tau_{n}$ and \ineq{\mathbf{t_k} = \{t_0(k),t_1(k),\cdots,t_8(k)\}}. 

Following definitions are introduced to estimate throughput.

\begin{Definition}{{Digraph}}
	The digraph $\Gamma(T)$ of a $n\times n$ matrix $T$ with entries defined in $\mathbb{R}_{\text{max}}$ is the tuple $\langle A,E\rangle$, where $A$ is the set of vertices, i.e., $A = \{1,2,\cdots n\}$ and $E$ is the set of connected ordered arcs between vertices i.e., $E = \{(i,j)~|~T_{i,j}\neq -\infty\}$.
\end{Definition}

\begin{Definition}{{Walk}}
	A walk $w$ in digraph $\Gamma(T)$ is the sequence of arcs $(x_1,x_2)(x_2,x_3)\cdots(x_{k-1},x_k)$;  head of an arc in the sequence is either the start vertex of the walk or tail vertex of a preceding arc; and the tail vertex of an arc in the sequence is either the end vertex of the walk or head vertex of a succeeding arc. Weight of the walk is given by
	\begin{equation}
	\label{eq:weight}
	\footnotesize|w|_T =  T_{x_1 x_2} + \cdots T_{x_{k-1} x_k}
	\end{equation}
\end{Definition}
\begin{Definition}{{Cycle}}
	A cycle $c$ in digraph $\Gamma(T)$ is the walk $(x_1,x_2)(x_2,x_3)\cdots(x_{k-1},x_k)$, such that $x_k = x_1$.
\end{Definition}
\begin{Definition}{{Maximum Cycle Mean}}
	The maximum cycle mean, $\rho_\text{max} (T)$ is the maximum of the weight-to-length ratio of all cycles $c$ in $\Gamma(T)$ i.e.,
	\mr{
	\begin{equation}
	\label{eq:mcm}
	\footnotesize\rho_\text{max} (T) = \max\limits_{\forall c \text{ in }\Gamma(T)}\frac{|c|_T}{|c|} = \max\limits_{k > 1} \max\limits_{x_1,\cdots,x_{k-1}} \frac{T_{x_1 x_2} + \cdots T_{x_{k-1} x_k}}{k-1}
	\end{equation}
	}
	%An alternative technique to compute the maximum cycle mean is using spectral analysis \cite{cochet1998numerical}.
\end{Definition}


Throughput of an SDFG is measured as the inverse of its \textit{maximum cycle mean} (Equation~\ref{eq:mcm}), i.e.,
\begin{equation}
    \label{eq:perf_def}
    \footnotesize \text{Performance (throughput)} = \frac{1}{\rho_\text{max} (T)}
\end{equation}

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/sdfg_example.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{(a) Projection block of ResNet with max pooling (POOL), convolution (CONV), batch normalization (BN), and addition (ADD) operations. (b) SDFG representation of the projection block. (c) Iterations of ResNet.}
	%\vspace{-10pt}
	\label{fig:sdfg_example}
\end{figure}

\subsection{Latency Characterization and SDFG Representation}
In our design flow, we represent an SDCNN as an SDFG, where an actor represents a layer (i.e., a specific operation of the model). Here, we discuss how the model can be characterized to extract the execution time of each layer. 
%(i.e., actor in SDFG terminology).
We consider each SDCNN operation can be implemented on the GPP and additionally on the NPU, if the NPU has the hardware to accelerate this operation.
Therefore, the execution time \ineq{\tau_i} of actor \ineq{\actor{a}_i\in A} is a tuple \ineq{\langle\tau_i^{G},\tau_i^{N}\rangle}, where \ineq{\tau_i^{G}} (\ineq{\tau_i^{N}}) is the time to perform the operation on the GPP (NPU) of the \nsoc{} platform.
This representation can be easily extended to consider several different types of computing units -- CPUs, GPUs, and flavors of NPUs.

We characterize SDCNN models to extract the execution time of their operations. 
Figure~\ref{fig:profile} shows the execution time (latency) of operations in the ResNet model on the GPP and NPU of the Akida \nsoc{}.
We make three key observations.

\begin{figure}[h!]
	\centering
	%\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/profile.pdf}}
	%\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Latency of different operations of ResNet, normalized to the latency of input processing on the NPU.}
	%\vspace{-10pt}
	\label{fig:profile}
\end{figure}

First, latency of each operation on the GPP is higher than on the NPU of the hardware by average 2.78x. 
Although the exact numerical value may differ, the trend is expected to be the same when the model is characterized for other \nsoc{} platforms.
Second, convolution (Conv) and perceptron (Dense) are compute-intensive operations compared to zero padding and max pooling.
This is why most neuromorphic research works focus on accelerating the matrix multiplication operation (e.g., using a crossbar) as it is a fundamental computation in these operations.
Third, an SDCNN may also have high-latency operations such as batch normalization and global average pooling. 
If the hardware acceleration of these operations are not possible (i.e., the NPU does not have the corresponding hardware), then this operation must be scheduled efficient on the GPP. This is exactly what we enable using our design flow.
%it is important to schedule these operations intelligently on the CPU to minimize the overall inference latency (and maximize the throughput).

These three observations are made for all fourteen evaluated SDCNN models (see Section~\ref{sec:evaluation}). The characterized data is then used to construct their SDFGs.




Algorithm~\ref{alg:profiler} shows the pseudo-code of one possible technique to extract the latency of each layer. 
This pseudo-code is based on Keras with TensorFlow backend.
Following are the steps of this algorithm.
First, a TensorFlow callback is defined to record the time it takes to process each batch (lines 1-7).
Second, the callback is instantiated (line 8) for use during the latency profiling.
Third, the target SDCNN model is loaded (line 9). We use serialized format where the model architecture is saved as a \texttt{json} file and weights as an \texttt{h5} file.
%We note that, the proposed methodology is independent of the exact method how the timing characteristics are obtained.

\begin{algorithm}[h]
	\scriptsize{
 		%\KwIn{\ineq{G_{SDCNN}= (\textbf{N},\textbf{E})}}
 		%\KwOut{\ineq{G_{DFG}= (\textbf{S},\textbf{C})}}
 		\Class(\tcc*[r]{Callback.}){\texttt{TimeHistory(callbacks.Callback)}}
 		{
 		    \Def{\texttt{on\_train\_begin(self, logs=\{\})}}
 		    {
 		        \texttt{self.times = []}\tcc*[r]{Start record.}\;
 		    }
 		    \Def{\texttt{on\_train\_batch\_end(self, logs=\{\})}}
 		    {
 		        \texttt{self.times.append(time.time() - self.epoch\_time\_start)}\tcc*[r]{End record.}
 		    }
 		
 		}
 		\texttt{time\_callback = TimeHistory()}\tcc*[r]{Instantiate.}
 		\texttt{model = load\_nodel(model\_name)}\tcc*[r]{Load the model.}
 		\texttt{os.environ["NPU\_VISIBLE\_DEVICES"] = 1/0}\tcc*[r]{To enable profiling on NPU (1) or GPP (0).}
 		\texttt{model.compile(loss=loss, optimizer=optimizer, metrics=[metrics])}\tcc*[r]{Compile the model.}
 		    \texttt{model.fit(x\_train, y\_train, batch\_size=batch\_size, epochs=epochs, validation\_data=(x\_val, y\_val), callbacks =[time\_callback])}\tcc*[r]{Train model.}
 		\texttt{base\_latency = np.average(time\_callback.times)}\tcc*[r]{Base latency.}
 		\texttt{latency = []}\tcc*[r]{list to store latencies.}
%  		\For(\tcc*[f]{For each layer}){$l\in \texttt{model.layers}$}{
%  		    $l.\texttt{trainable}$ = \textbf{False}\tcc*[r]{Set layer as non-trainable.}
%  		}* $\eta$ / batch\_size) * $\eta$ / batch\_size)
 		\For(\tcc*[f]{For each layer}){$l\in \texttt{model.layers}$}{
 		    $l.\texttt{trainable}$ = \textbf{False}\tcc*[r]{Set layer as non-trainable.}
 		    \texttt{model.compile(loss=loss, optimizer=optimizer, metrics=[metrics])}\tcc*[r]{Compile the model.}
 		    \texttt{model.fit(x\_train, y\_train, batch\_size=batch\_size, epochs=epochs, validation\_data=(x\_val, y\_val), callbacks =[time\_callback])}\tcc*[r]{Train model.}
 		    \texttt{latency.append(np.average(time\_callback.times)}\tcc*[r]{Latency without the layer.}
 		}
 		\texttt{latency = base\_latency - latency}\tcc*[r]{Layer latency.}
 		\texttt{latency = latency * $\eta$ / batch\_size}\tcc*[r]{Inference latency.}
 	}
	\caption{\footnotesize{Profiling the latency of each layer of an SDCNN.}}
	\label{alg:profiler}
\end{algorithm}

Four, the model is compiled and trained (lines 11-12) using training data for the specific batch size and number of epochs.
The base latency is computed (line 13).
Finally, for each layer of the model, the algorithm sets its trainable parameter to \texttt{False} (line 16). Subsequently, it compiles the model (line 17), trains the model (line 18), and record the latency (line 19).
This is the latency of the model without training the layer.
Therefore, to compute the latency introduced by the layer we subtract these latencies from the base latency (line 20).
Unfortunately, Keras callbacks report the total latency for each batch, which includes 1) latency for forward-pass (\ineq{\approx} 25\%), 2) latency for backward-pass (\ineq{\approx} 70\%), and 3) latency for parameter optimization (\ineq{\approx} 5\%). 
These distributions are specific to the Akida \nsoc{} platform.
Therefore, to compute the inference latency we use only 25\% of the obtained latencies, which is represented by the parameter \ineq{\eta} in line 21 of the algorithm.
For other platforms, \ineq{\eta} needs to be set differently.
We divide these latencies with the batch size to compute the inference latency per image.
By setting the OS environment \texttt{NPU\_VISIBLE\_DEVICES} to 1 and 0 (line 10), profiling can be enabled for NPU and GPP, respectively.

Algorithm~\ref{alg:profiler} is one possible technique to compile the inference latency for each layer of a model. Alternatively, TensorBoard can also be used to do such profiling. 
In~\cite{zhao2016f}, authors report layer profiling for FPGA-based model implementation.
Therefore, any of these existing solutions may also be used in our design flow to construct the SDFG.
